PolicyGuide: From Guarding One Action to Guiding the Whole Workflow for Policy-Compliant LLM Agents

Customer-service LLM agents must follow organizational policy when acting on a user's behalf. Compliance failures arise from either forbidden actions, such as granting an ineligible change, or omitted procedural requirements, such as identification or confirmation. Runtime safeguards can intervene on risky actions, but action-local checks do not guide an agent through a multi-step procedure. Workflow-following systems support prescribed process execution, but primarily target workflow completion rather than safeguarding agent behavior. PolicyGuide instead compiles each domain policy into a workflow graph and invokes a proactive verifier at user-turn boundaries. From persisted graph state, the verifier reconciles open requests and returns step-specific remediation along a policy-compliant path. Across the $\tau^2$-bench airline, retail, and telecom domains with a GPT 5.4 agent and verifier, PolicyGuide raises mean $\mathrm{Pass}^4$ from $0.42$ to $0.62$, with the largest gain on telecom ($0.19$ to $0.61$), the most workflow-structured domain. The same workflows transfer to Claude Sonnet 4.6 and Gemini 2.5 Pro agents. Complementary evaluations find the lowest observed attack-success rate under adversarial users and the strongest procedural compliance in an independently validated workflow-level audit.

==> sections/A08_confusion_analysis.tex <==
\section{Per-call verdict diagnostic}
\label{app:confusion}

We apply \pgd{}'s verdict convention~\citep{kang2026policyguard} to every
attempted agent-side mutating tool call. Each call inherits its task label:
PV is positive and Mut is negative; a block is a positive prediction and a
passed call is negative. Thus TP/FN are blocked/passed calls on PV tasks, and
FP/TN are blocked/passed calls on Mut tasks. Because this task-slice label does
not judge the specific call and retries count separately, the result diagnoses
the fallback gate rather than semantic call correctness.

\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrr}
\toprule
Domain & PV sims & \makecell{PV sims\\with call} &
\makecell{PV calls\\B/P} & \makecell{Mut calls\\B/P} & PV Pass$^1$ \\
\midrule
\tblairlinedomain{} & 96  & 3  & 0/3  & 10/180 & 94/96 \\
\tblretaildomain{}  & 40  & 1  & 0/1  & 79/660 & 39/40 \\
\tbltelecomdomain{} & 172 & 19 & 6/31 & 35/377 & 154/172 \\
\midrule
Micro & 308 & 23 & 6/35 & 124/1,217 & 287/308 \\
\bottomrule
\end{tabular}%
}
\caption{Mutation-call exposure and fallback-gate outcomes ($n{=}4$).
B/P denotes blocked/passed attempted calls; PV Pass$^1$ is end-to-end.}
\label{tab:call-diagnostic}
\end{table}

The zero Airline and Retail TP counts mean that the fallback gate blocks none
of the three and one PV calls that reach it, respectively---not that \pg{}
prevents no violations. No mutation call is proposed in the other 93 Airline
and 39 Retail PV simulations, which therefore never enter a call-level
confusion matrix; end-to-end PV Pass$^1$ remains $94/96$ and $39/40$. Telecom
exposes 37 PV calls from 19 simulations and blocks six.

Across domains, the gate therefore blocks $6/41$ exposed PV calls. This
conditional rate describes residual calls after proactive guidance, not overall
prevention. Moreover, the one-shot gate disarms for a corrective retry, so one
simulation may contribute both a block and a pass. We omit a cross-system
confusion table because \pgd{} uses an always-on call-level schedule, whereas
\pg{} primarily intervenes upstream; their exposed calls and retry counts are
not paired comparison units.


==> tabs/taxonomy.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccc}
\toprule
System & Mechanism & Context scope & Conv. & Reason & Remed. & \textbf{Workflow} \\
\midrule
\tg{} \citep{zwerdling2025toolguard}    & Python guards       & tool arguments     & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
Solver-Aided \citep{winston2026solver}  & Z3 / SMT            & tool arguments     & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
PCAS \citep{palumbo2025pcas}            & Datalog monitor     & event DAG + text   & \ding{51} & \ding{55} & \ding{55} & \ding{55} \\
ShieldAgent \citep{chen2025shieldagent} & LTL rule circuits   & action sequence    & part.     & \ding{55} & \ding{55} & \ding{55} \\
GuardAgent \citep{xiang2025guardagent}  & LLM $\to$ code      & single $(I,O)$     & \ding{55} & part.     & \ding{55} & \ding{55} \\
AgentSpec \citep{wang2026agentspec}     & DSL predicates      & state + actions    & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
ToolSafe \citep{mou2026toolsafe}        & RL guard model      & current request    & \ding{55} & \ding{55} & part.     & \ding{55} \\
\nemo{} \citep{rebedea2023nemo}         & Colang flows        & dialogue (scripted)& part.     & \ding{55} & \ding{55} & \ding{55} \\
\pgd{} (predecessor)                    & LLM verifier        & full conversation  & \ding{51} & \ding{51} & \ding{51} & \ding{55} \\
\rowcolor{ourrowbg}
\textbf{\pg{} (ours)}                    & \textbf{workflow guide} & \textbf{full conv.\ + graph position} & \ding{51} & \ding{51} & \ding{51} & \textbf{\ding{51}} \\
\bottomrule
\end{tabular}%
}
\caption{Capability taxonomy of runtime safeguards. \emph{Conv.}: reads the
user--agent conversation; \emph{Reason}: open semantic reasoning over policy in
context; \emph{Remed.}: conversation-specific remediation; \emph{Workflow}: enforces
the full multi-step procedure (reads, agent turns, confirmation gates) rather than
only the final mutating call. Every prior system---including our predecessor
\pgd{}---is action-scoped; \pg{} is the only workflow-scoped safeguard.}
\label{tab:taxonomy}
\end{table*}


==> tabs/test.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{llr ccc ccc ccc}
\toprule
& & & \multicolumn{3}{c}{\direct{}} & \multicolumn{3}{c}{\pgd{}} & \multicolumn{3}{c}{\cellcolor{ourrowbg}\textbf{\pg{}}} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
Domain & Split & $n$ & Overall & PV & Mut & Overall & PV & Mut & \cellcolor{ourrowbg}Overall & \cellcolor{ourrowbg}PV & \cellcolor{ourrowbg}Mut \\
\midrule
\multirow{3}{*}{\airlinedomain}
 & Train & 30  & 0.500 & 0.706 & 0.231 & 0.633 & \textbf{1.000} & 0.154 & \cellcolor{ourrowbg}\textbf{0.667} & \cellcolor{ourrowbg}0.882 & \cellcolor{ourrowbg}\textbf{0.385} \\
 & Test  & 20  & 0.400 & 0.857 & 0.154 & 0.500 & \textbf{1.000} & 0.231 & \cellcolor{ourrowbg}\textbf{0.550} & \cellcolor{ourrowbg}\textbf{1.000} & \cellcolor{ourrowbg}\textbf{0.308} \\
 & Base  & 50  & 0.460 & 0.750 & 0.192 & 0.580 & \textbf{1.000} & 0.192 & \cellcolor{ourrowbg}\textbf{0.620} & \cellcolor{ourrowbg}0.917 & \cellcolor{ourrowbg}\textbf{0.346} \\
\midrule
\multirow{3}{*}{\retaildomain}
 & Train & 74 & \textbf{0.608} & \textbf{0.750} & \textbf{0.600} & 0.554 & \textbf{0.750} & 0.543 & \cellcolor{ourrowbg}0.554 & \cellcolor{ourrowbg}\textbf{0.750} & \cellcolor{ourrowbg}0.543 \\
 & Test & 40 & 0.575 & \textbf{1.000} & 0.541 & 0.550 & \textbf{1.000} & 0.514 & \cellcolor{ourrowbg}\textbf{0.725} & \cellcolor{ourrowbg}\textbf{1.000} & \cellcolor{ourrowbg}\textbf{0.703} \\
 & Base & 114 & 0.596 & \textbf{0.857} & 0.579 & 0.605 & \textbf{0.857} & 0.589 & \cellcolor{ourrowbg}\textbf{0.614} & \cellcolor{ourrowbg}\textbf{0.857} & \cellcolor{ourrowbg}\textbf{0.598} \\
\midrule
\multirow{3}{*}{\telecomdomain}
 & Train & 74  & 0.162 & 0.455 & 0.038 & 0.135 & 0.364 & 0.038 & \cellcolor{ourrowbg}\textbf{0.581} & \cellcolor{ourrowbg}\textbf{0.773} & \cellcolor{ourrowbg}\textbf{0.500} \\
 & Test  & 40  & 0.250 & 0.429 & 0.053 & 0.325 & 0.619 & 0.000 & \cellcolor{ourrowbg}\textbf{0.675} & \cellcolor{ourrowbg}\textbf{0.667} & \cellcolor{ourrowbg}\textbf{0.684} \\
 & Base  & 114 & 0.193 & 0.442 & 0.042 & 0.202 & 0.488 & 0.028 & \cellcolor{ourrowbg}\textbf{0.614} & \cellcolor{ourrowbg}\textbf{0.721} & \cellcolor{ourrowbg}\textbf{0.549} \\
\bottomrule
\end{tabular}
\caption{Train/test decomposition of the base-split results (\gptfive{} agent,
$n{=}4$). Airline uses 30/20 train/test tasks; Retail and Telecom use 74/40.
Base is their disjoint union. All cells report Pass$^4$.}
\label{tab:test}
\end{table*}

